Using Graph-Aware Reinforcement Learning to Identify Winning Strategies in Diplomacy Games (Student Abstract)

This abstract proposes an approach towards goal-oriented modeling of the detection and modeling complex social phenomena in multiparty discourse in an online political strategy game. We developed a two-tier approach that first encodes sociolinguistic behavior as linguistic features then use reinforcement learning to estimate the advantage afforded to any player. In the first tier, sociolinguistic behavior, such as Friendship and Reasoning, that speakers use to influence others are encoded as linguistic features to identify the persuasive strategies applied by each player in simultaneous two-party dialogues. In the second tier, a reinforcement learning approach is used to estimate a graph-aware reward function to quantify the advantage afforded to each player based on their standing in this multiparty setup. We apply this technique to the game Diplomacy, using a dataset comprising of over 15,000 messages exchanged between 78 users. Our graph-aware approach shows robust performance compared to a context-agnostic setup.

==> tables/dataset.tex <==
\begin{table}[!h]
\caption{Stratified split for the two datasets}
\label{tab:traintestpolarity}
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{lrrrr}
\hline
\multirow{2}{*}{\textbf{Dataset - Variable}} & \multicolumn{2}{c}{\textbf{Training}} & \multicolumn{2}{c}{\textbf{Testing}} \\ 
& 1 & 0 & 1 & 0 \\ \hline
Diplomacy - Deception & 8646 & 446 & 2162 & 112\\ \hline
%Diplomacy - Rapport & 7823& 1269 & 1981& 293\\ \hline
CLAff-OffMyChest - Popularity & 11403& 2575& 2851& 644\\ \hline
\end{tabular}
}
\end{center}
\end{table}

==> tables/diplomacyannotation.tex <==
\vspace*{-\baselineskip}
\begin{table}[!ht]
\caption{CLAff-Diplomacy dataset labels.}
\label{tab:diplomacyannotation}
\begin{center}
\small
 \resizebox{0.45\textwidth}{!}{
\begin{tabular}{p{1cm}p{3cm}p{5cm}}
\hline
\textbf{Label} & \textbf{Elaboration} & \textbf{Example message} \\ \hline
%Deception & Whether or not the receiver thinks the speaker is lying & ``I think I can top Germanys offer if youre interested." \newline
%``I want it to be clear to you that youre the ally I want."\\
%\hline
Friendship & Build rapport & ``I won't hold it against you"\\ %\newline ``I'm going to keep helping you as much as I can." \\ \hline
Reasoning & Justify a move & ``If you took Marseilles, I would be stronger against England"\\% \newline ``France is a really good player, and he is no doubt working hard to get England to turn on you."\\ 
\hline
Game Move & Actual or suggested game move & ``I am committed to supporting Munich holding" %\newline ``Make sure you don't move Munich so that it can take my support." 
\\ \hline
Share Information & Share information related to other players & ``France is a really good player, and he is no doubt working hard to get England to turn on you." %\newline ``And anything that's bad for Russia right now is good for Austria."
\\ \hline
\end{tabular}
}
\end{center}
\end{table}
\vspace*{-\baselineskip}


==> tables/diplomacyannotationfiltered.tex <==
\begin{table}[!ht]
\caption{CLAff-Diplomacy labels.}
\label{tab:diplomacyannotation}
\begin{center}
\small
 \resizebox{0.5\textwidth}{!}{
\begin{tabular}{p{1cm}p{3cm}p{5cm}}
\hline
\textbf{Label} & \textbf{Elaboration} & \textbf{Example \newline Messages} \\ \hline
Friendship & Exchanges or information that propel friendship between two players & ``Just letting a friend know so that you can bounce him." \newline
``I'm willing to help you switch your focus to AH and Italy, and even help you eventually but we need to build the trust before I decommission the fleet in Black Sea I think."\\
\hline
Reasoning & Justify a move, guess what moves might happen next, or discuss a move that already happened & ``If you took Marseilles, I would be stronger against England" \newline ``France is a really good player, and he is no doubt working hard to get England to turn on you."\\ \hline
Game Move & Actual or suggested game move & ``I am committed to supporting Munich holding" \newline ``Make sure you don't move Munich so that it can take my support." \\ \hline

Share Information & Share information related to other players & ``France is a really good player, and he is no doubt working hard to get England to turn on you." \newline ``And anything that's bad for Russia right now is good for Austria."\\ \hline

\end{tabular}
}
\end{center}
\end{table}



==> tables/diplomacyannotationfull.tex <==
\begin{table}[!ht]
\caption{CLAff-Diplomacy labels.}
\label{tab:diplomacyannotation}
\begin{center}
\small
 \resizebox{0.5\textwidth}{!}{
\begin{tabular}{p{1cm}p{3cm}p{5cm}}
\hline
\textbf{Label} & \textbf{Elaboration} & \textbf{Example \newline Messages} \\ \hline
Deception & Whether or not the receiver thinks the speaker is lying & ``I think I can top Germanys offer if youre interested." \newline
``I want it to be clear to you that youre the ally I want."\\
\hline
Game Move & Actual or suggested game move & ``I am committed to supporting Munich holding" \newline ``Make sure you don't move Munich so that it can take my support." \\ \hline
Reasoning & Justify a move, guess what moves might happen next, or discuss a move that already happened & ``If you took Marseilles, I would be stronger against England" \newline ``France is a really good player, and he is no doubt working hard to get England to turn on you."\\ \hline
Share Information & Share information related to other players & ``France is a really good player, and he is no doubt working hard to get England to turn on you." \newline ``And anything that's bad for Russia right now is good for Austria."\\ \hline
Rapport & Build rapport through compliments, concerns, reassurances or apologies & ``I won't hold it against you" \newline ``I'm going to keep helping you as much as I can." \\ \hline
\end{tabular}
}
\end{center}
\end{table}



==> tables/indiv.tex <==
\begin{table}[!htb]
\caption{\small Macro-F1 scores for feature estimators}
 \vspace{-\baselineskip}
\vspace{0.1cm}
\label{tab:individualscoresdataset1}
\begin{center}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{l r r r r r r}

\hline

& \textbf{Friendship} & \textbf{Reasoning} & \textbf{Game Move}  & \textbf{Share Information}\\ \hline
Logistic Regression & 0.633 & 0.508 & 0.695 & 0.541 \\ 
KNN & 0.587 & 0.484 & 0.566 & 0.517 \\ 
Gaussian NB & 0.467 & \textbf{0.533} & 0.620 & 0.315 \\ 
Bernoulli NB & 0.611 & 0.517 & 0.646 & 0.547 \\ 
Adaboost & 0.642 & 0.448 & 0.696 & \textbf{0.623} \\ 
Gradient Boosting & 0.641 & 0.445 & \textbf{0.698} & 0.611 \\ 
Decision Tree & 0.615 & 0.511 & 0.624 & 0.591 \\ 
Linear SVC & 0.636 & 0.516 & 0.697 & 0.563 \\ 
C-SVC & \textbf{0.673} & 0.526 & 0.692 & 0.570 \\ 
LDA & 0.641 & 0.446 & 0.686 & 0.599 \\ 

% & \textbf{Friendship} & \textbf{Reasoning} & \textbf{Game Move} & \textbf{My Move }  & \textbf{Your Move} & \textbf{Other Move}\\ \hline
% Logistic Regression & 0.624 & 0.512 & 0.694 & \textbf{0.681} & 0.685 & 0.551 \\ 
% KNN & 0.570 & 0.471 & 0.601 & 0.574 & 0.629 & 0.496 \\ 
% Gaussian NB & 0.419 & \textbf{0.531} & 0.629 & 0.532 & 0.616 & 0.350 \\ 
% Bernoulli NB & 0.607 & 0.520 & 0.642 & 0.635 & 0.676 & 0.544 \\ 
% Adaboost & 0.624 & 0.452 & 0.684 & 0.643 & 0.693 & \textbf{0.613} \\ 
% Gradient Boosting & 0.638 & 0.449 & 0.698 & 0.653 & \textbf{0.707} & 0.606 \\ 
% Decision Tree & 0.603 & 0.502 & 0.644 & 0.600 & 0.643 & 0.575 \\ 
% Linear SVC & 0.627 & 0.524 & 0.695 & 0.678 & 0.688 & 0.560 \\ 
% C-SVC & \textbf{0.670} & 0.524 & \textbf{0.707} & 0.680 & 0.692 & 0.570 \\ 
% LDA & 0.632 & 0.444 & 0.696 & 0.650 & 0.701 & 0.591 \\ 
\hline
\end{tabular}
}
\end{center}

\end{table}
